Neural network based deep learning analysis of semiconductor quantum dot qubits for automated control

Machine learning offers a largely unexplored avenue for improving noisy disordered devices in physics using automated algorithms. Through simulations that include disorder in physical devices, particularly quantum devices, there is potential to learn about disordered landscapes and subsequently tune devices based on those insights. In this work, we introduce a novel methodology that employs machine learning, specifically convolutional neural networks (CNNs), to discern the disorder landscape in the parameters of the disordered extended Hubbard model underlying the semiconductor quantum dot spin qubit architectures. This technique takes advantage of experimentally obtainable charge stability diagrams from neighboring quantum dot pairs, enabling the CNN to accurately identify disorder in each parameter of the extended Hubbard model. Remarkably, our CNN can process site-specific disorder in Hubbard parameters, including variations in hopping constants, on-site potentials (gate voltages), and both intra-site and inter-site Coulomb terms. This advancement facilitates the prediction of spatially dependent disorder across all parameters simultaneously with high accuracy ($R^2>0.994$) and fewer parameter constraints, marking a significant improvement over previous methods that were focused only on analyzing on-site potentials at low coupling. Furthermore, our approach allows for the tuning of five or more quantum dots at a time, effectively addressing the often-overlooked issue of crosstalk. Not only does our method streamline the tuning process, potentially enabling fully automated adjustments, but it also introduces a "no trust" verification method to rigorously validate the neural network's predictions. Ultimately, this work aims to lay the groundwork for generalizing our method to tackle a broad spectrum of physical problems.

==> Sup.tex <==
\begin{bibunit}
\clearpage
\pagebreak
\widetext
\begin{center}
\textbf{\large Supplemental Materials: Machine learning Majorana nanowire disorder landscape}
\end{center}
%%%%%%%%%% Merge with supplemental materials %%%%%%%%%%
%%%%%%%%%% Prefix a "S" to all equations, figures, tables and reset the counter %%%%%%%%%%
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{1}
\makeatletter
\makeatother
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\bibnumfmt}[1]{[S#1]}
\renewcommand{\citenumfont}[1]{S#1}
\setcounter{section}{0}
\renewcommand{\thesection}{S-\Roman{section}}
\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
\section{Details of theory}
We model the 1D semiconductor Majorana nanowire using a Bogoliubov-de Gennes  Hamiltonian \cite{lutchyn2010majorana}:
\begin{equation}
H=\left( -\frac{\hbar^2}{2m^*}\partial_x^2-i\alpha \partial_x \sigma_y - \mu +V_{\text{dis}}(x) \right)\tau_z\\ +\frac{1}{2}g \mu_B B\left(\sigma_x\cos\theta+\sigma_y\sin\theta \right)+\Sigma(\omega)
\label{eqn:1}
\end{equation}
where $$\Sigma(\omega)=-\gamma \frac{\omega+\Delta_0\tau_x}{\sqrt{\Delta_0^2-\omega^2}}$$ is the self-energy generated by integrating out the superconductor that is proximity coupled to the semiconductor~\cite{sau2010robustness}. The above Hamiltonian is a $4\times4$ matrix comprised of $\sigma_{x,y,z}$, which are $2\times2$ Pauli matrices associated 
with the spin degree of freedom, and $\tau_{x,y,z}$, which are $2\times2$ Pauli matrices associated with the superconducting particle-hole degree of freedom. The above Hamiltonian is written in a basis where the Bogoliubov quasiparticles of the superconductor are described by a Nambu spinor with a structure $\psi(x)=(u_{\uparrow}(x), u_{\downarrow}(x),-v_{\downarrow}(x),v_{\uparrow}(x))^T$, where $\uparrow,\downarrow$ refer to spin and $u,v$ refer to particle-hole components of the quasiparticle. The frequency $\omega$ in the self-energy is equivalent to the energy (in units where $\hbar=1$) of the Bogoliubov quasiparticle in consideration. While, this requires a self-consistent solution for eigenstates in a closed system, the $\omega$ dependence of $\Sigma$ does not present any additional complication in the solution of transport problems in open systems using KWANT~\cite{groth2014kwant}. Specifically, KWANT solves the transport problem of the Majorana nanowire by computing the scattering matrix of the system in the particle-hole space between the two leads shown in Fig.~\ref{fig:DeviceSketch}. 
The scattering matrix can be used to compute the conductance matrix $G_{\alpha\beta}$ using the well-known Blonders-Tinkham-Klapwijk relations~\cite{groth2014kwant}. In addition, one can use the reflection matrix from either of the lead ends to compute the topological visibility $T_{IV}$~\cite{akhmerov2011quantized,pan2021three}.

The actual semiconductor device is a complicated three dimensional semiconductor system. Despite this, the transport properties computed by KWANT \cite{groth2014kwant} using the model Hamiltonian Eq.~\ref{eqn:1} captures most qualitative features of the transport properties of the device over the relevant ranges of gate and bias voltages provided the parameters $\alpha$, $\mu$ etc are taken to be fitting parameters. Therefore, the parameters $m^*$, $\alpha$, $\ldots$ should ideally be viewed as fitting parameters to transport properties of devices. In practice~\cite{pan2021three,woods2021charge,sarma2023spectral}, the parameters such as effective mass $m^*=0.03 m_e$ and a nominal (details later) value of the spin-orbit coupling $\alpha=8.0\,meV-nm$ are chosen to fit non-superconducting transport characterization of the InAs nanowire device. The superconducting pairing potential coupling parameter $\gamma=0.15\,meV$, the Lande g-factor $g=25$ are chosen to qualitatively reproduce transport properties in the superconducting phase. The intrinsic superconducting pair potential $\Delta_0=0.12\,meV$ is chosen according to be the superconducting gap of the Al superconductor. In addition, to model transport in the system given by the Hamiltonian in Eq.~\ref{eqn:1}, we choose a temperature $T=50mK$, and device length $L=3\,\mu m$. 
%$V_{\text{Bias}}$ is a special parameter because we do not have the flexibility of only generating $V_{\text{Bias}}$ values that we will use within the machine learning model.
The finite temperature is implemented in the system by convolving the zero temperature conductance as a function of $\omega$ with the derivative of a Fermi function at temperature $T$. For this purpose, we generate the zero-temperature conductance using KWANT at an $\omega$ grid with 151 points between $\pm 0.04$ meV. 
Finally, for the purpose of numerical simulations we discretize the Hamiltonian in Eq.~\ref{eqn:1} with a lattice scale of a=10 nm. These parameters are chosen from recent work \cite{sarma2023spectral}, which was focused on understanding the recent experiments from the Microsoft group \cite{aghaee2023inas}. 

 The disorder potential generated by impurities in the device is also included in the Hamiltonian $H$ through the function 
 $V_{\text{dis}}(x)$. The spatial disorder potential is assumed to  randomly varying with position $x$ across the length of the wire with a Gaussian distribution with an amplitude $1.5\,\text{meV}$ and correlation length of $30\,nm$. 
 For the purposes of simplifying the ML complexity by reducing the number of parameters, we eliminate (i.e. set to 0) all but $N_{dis}$ of the Fourier components of the disorder potential. For our calculations we will use $N_{dis}=5$ or $10$.
 In addition,
we also include barrier potentials $V_{\text{Barrier}}^L$ and $V_{\text{Barrier}}^R$ as $\delta$ function contributions at the ends of the wire to $V_{\text{dis}}(x)$. 


Out of the parameters that go into $H$, the spacial profile of the disorder potential $V_\text{dis}(x)$, which  is specified in our model by the $N_{dis}$ Fourier components, is completely uncontrolled and varies between devices as well as slowly over time. In addition, some parameters such as $\alpha$ depend on the inversion symmetry breaking of the final device structure, where it is difficult to interpret the transport data.
%Therefore till now it has been impossible to perform a quantitative simulation of any disorder potential. 
In this work, we will vary the disorder potential and spin-orbit coupling $\alpha$  (around the aforementioned nominal value) to generate, using KWANT, training transport data set as a function of  chemical potential $\mu$, magnetic field  $B$ and bias voltage $V_{bias}$ (related to $\omega$ in $H$) to be fit by an ML algorithm. To keep the computation in this work simple, we assume the other parameters in the Hamiltonian $H$ are fixed at values estimated from experiment. The ML algorithm will then predict the Fourier components of $V_\text{dis}$ and spin-orbit coupling $\alpha$ from transport  that can be used using KWANT to match a test transport data. Ideally, the test transport data would come from experiment though that would likely require more fit parameters. In our proof of principle demonstration, our test transport data is generated using KWANT using a random choice of disorder configuration and $\alpha$. 



%We will however in one of our models vary $\alpha$. These parameters are used to generate a

\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{DeviceSketch.png}
         \caption{}
         \label{fig:S1b}
     \end{subfigure}
     \caption{Sketch of Majorana nanowire device. The device consists of a NS junction with a layer of superconductor on top of a layer of semiconductor, with opposite ends of the semiconductor connected to left and right leads respectively \cite{pan2020physical}. The differential conductances, which are measured, are defined as $G_{\alpha \beta}= dI_\alpha/dV_\beta$ for $\alpha =\beta$ and $G_{\alpha \beta}= -dI_\alpha/dV_\beta$ for $\alpha \neq \beta$. Local conductances $G_{LL}$ and $G_{RR}$ are measured from their respective leads through the junction (to the superconductor), while non-local conductances $G_{RL}$ and $G_{LR}$ are measured from the right lead to the left lead or the reverse respectively.}
     \label{fig:DeviceSketch}
\end{figure*}

\section{Details of Machine Learning}
\label{S:ML}
\subsection{Training Data}
The training data was generated within KWANT for many different randomly generated $V_\text{dis}(x)$ and $\alpha$ configurations (called Y realizations). For each Y realization we calculate a set of $G_{\text{RR}}$, $G_{\text{LL}}$, $G_{\text{RL}}$, $G_{\text{LR}}$ values for different measurement configurations. A Y realization consists of generating a random $\alpha$ from a uniform distribution between 6.4 and 9.6, along with a random Gaussian disorder potential. The disorder potential $V_\text{dis}(x)$ refers to disorder within the $\mu$ chemical energy taking $\mu \rightarrow \mu + V_{dis}(x)$.  The disorder potential is transformed with a discrete cosine transform, and only the nth lowest frequency components are kept. This gives us $c_1 ... c_n$, the transformed disorder potential components. The transformation is then undone to get the disorder potential in real space corresponding to these components. This truncated then reverse transformed $V_{dis}(x)$ is what will be used by KWANT. From the transformed components we define a vector for each Y realization:
$$Y=\begin{bmatrix}c_1 & \ldots & c_n & \alpha \end{bmatrix}$$
This is done for many different Y realizations, each time having the potential along with $\alpha$ numerically simulated to evaluate a sequence of conductance measurements. The measurement configurations were recorded in a matrix $K$ where each row would record a particular setup of experimentally tunable parameters labelled as j:

$$\textbf{K}_{\text{full}}=\begin{bmatrix}\mu^j & B^j & V^{L,j}_{\text{Barrier}} & V^{R,j}_{\text{Barrier}} &\theta^j& V^j_{\text{Bias}}\end{bmatrix}$$
where $B$ is the applied magnetic field, $\mu$ is the chemical potential parameter controlled by the plunger gate voltage, $V^L_{\text{Barrier}}$ and $V^R_{\text{Barrier}}$ are the left and right barrier voltages respectively, $\theta$ is the angle of the B field relative to the direction of the wire, and $V_{\text{Bias}}$ is the bias voltage. All these are parameters that are readily varied in a transport experiment. The Hamiltonian that is described 
in the previous section, which is used in the KWANT simulation contains all of these parameters except $\theta$,  which has been assumed to be zero for simplicity. The possibility of varying all these parameters to study transport provides the potential of generating a huge volume of transport data to characterize a specific device. In our case, we found it either unnecessary or beyond our limited computational resources to use transport data in the entire space to estimate the disorder in the device. As such we fixed $V^{L}_{\text{Barrier}}=V^{R}_{\text{Barrier}}=15$ meV and $\theta=0$. The simplified $\mathbf{K}$ we use is as follows:  

$$\textbf{K}=\begin{bmatrix}\mu^j & B^j & V^j_{\text{Bias}}\end{bmatrix}$$

Furthermore, $V_{\text{Bias}}$ turns out to not be necessary to fit the transport data when 5 disorder Fourier components are used. Therefore, in this case it is removed from the $K$ matrix and set to $V_{\text{Bias}}=0$. In contrast, the 10 Fourier component disorder models require more transport data to fit and in this case we include  $V_{\text{Bias}}$ in the $K$ matrix. For these calculations, $V_{\text{Bias}}$ takes one of two values  $V_{\text{Bias}}=0$ meV and 
$V_{\text{Bias}}=32\,\mu eV$ depending on the realization index $j$.
Each row of K when fed into KWANT generates a new set of conductance measurements, we put these conductances into a matrix we call $\textbf{X}$ as follows: 

$$\textbf{X}=\begin{bmatrix} G_{\text{RR}}^j& G_{\text{LL}}^j & G_{\text{RL}}^j & G_{\text{LR}}^j\end{bmatrix}$$


Putting this all together we get our training data generating function as follows: $$F_{\text{Gen}}(Y;\textbf{K})=\textbf{X}$$ 

Note that all the different Y realizations have the same K matrix. It can be seen then that our objective is to find a function that can take in $\textbf{X}$ and $\textbf{K}$, and give us $Y$. Put another way we wish to invert our generator function to find the following: 

$$F^{-1}_{ML}(\textbf{X};K)=Y$$


%The spacial disorder potential was generated, truncating it's components in frequency space with a discrete cossine transform, then transforming back to real space. Constant boundary effects were then added to modify the spacial disorder potential.

In terms of the other components, we varied $\mu$ between 0 meV and 0.6 meV (with 15 steps), $B_x$ between 0 T and 0.8 T (with 15 steps). Overall our $\textbf{K}$ matrix had 225*$N_{V_\text{Bias}}$ rows, as we do not feed all the $V_{\text{bias}}$ data into the neural network. $N_{V_\text{Bias}}=1$ and $N_{V_\text{Bias}}=2$ for 5 and 10 component versions respectively.

In summary we generate many random realizations of $V^i_\text{dis}(x)$ and $\alpha^i$, cosine transform each $V^i_\text{dis}(x)$ and truncate to either 5 or 10 components to form a $Y^i_\text{input}$. Using this we calculate $F_{\text{Gen}}(Y^i_\text{input};K) = X^i_\text{input}$, where within KWANT $Y^i_\text{input}$ is inverse cosine transformed back into real space. The $X_\text{input}^i$, $Y^i_\text{input}$ pairs are split between training $X_\text{train}^i$, $Y^i_\text{train}$ and testing $X_\text{test}^i$, $Y^i_\text{test}$.  Using $X_\text{train}^i$, $Y^i_\text{train}$ we train a neural network to be able to generate a prediction for $Y$ given an $\mathbf{X}$. We assess the validity of our model by comparing $Y^i_\text{test}$ to our neural network prediction $F_{ML}^{-1}(\mathbf{X}_\text{test}^i;K)=Y^i_\text{{Pred}}$. 

\subsection{The Neural Network}

Our machine learning model consisted of a recurrent neural network (RNN) created the package Keras \cite{chollet2015keras} which is a package that builds upon tensorflow \cite{tensorflow2015-whitepaper}. In the RNN each input step consisted of a measurement operation, 10 parameters consisting of a row of $\textbf{X}$ (4 parameters) and of $\textbf{K}$ (6 parameters). For this reason it is useful for us to define a combined measurement result matrix $\textbf{m}=[\textbf{X},\textbf{K}]$. A RNN was used so that the addition of more measurements would not decrease the ability of the previous measurements to perform predictions for a constant amount of training data. This is sub-optimal as RNNs are order dependent, while the order one performs the conductance measurements shouldn't matter. Ideally a convolution neural network (CNN) would be preferable, {\color{red}in particular, using a GPU based convolutional neural network architecture we are able to achieve a higher $R_2=0.884$ for the 10 component version of our scheme using the same $K$ matrix and only $V_{\text{Bias}}=0$}, however since our $\textbf{K}$ and thus measurement order is the same for all input an easier RNN was sufficient. In particular the RNN for the 5 disorder components and 1 alpha (5+1 component model) consisted of 3 GRU hidden recurrent layers with 150 nodes each, which were then followed up with a non-recurrent 100 node dense hidden layer. In the case of the 10 components model we instead had 5 GRU layers, still with 150 nodes each.  A figure of this can be seen in Fig. 1.



We measure the effectiveness of our model using the standard scaled $R_2$. This is calculated between $\{Y^i_\text{{test}}\}$ and $\{Y^i_\text{{Pred}}\}$. The standard scaling converts the data used in the training processes into a 0 mean, unit variance form. A $R_2=1$ implies perfectly predicting the tests, while $R_2=0$ is equivalent to just taking the average output of the testing data. This scaling and $R_2$ can be found within the package Scikit-learn \cite{pedregosa2011scikit}.



{\color{red} 
\subsection{Computational Resources and Scaling}
In terms of computational resources, the generation of training data proves to be significantly more demanding than the training process itself. Fortunately, the task of training data generation exhibits an "embarrassingly parallel" nature. Each set of $N_{V_{Bias}}$ rows in matrix K can be computed in parallel with minimal overhead. For our specific setup, generating conductance data for $N_{V_{Bias}}$ rows in K took approximately 12 seconds per set using a single core. With a total of 225 sets of rows and 50,000 different Y realizations, this amounts to a total processing time of 37.5 thousand core hours. Considering that many supercomputers boast tens of millions of cores, our approach can certainly be scaled up efficiently.

In contrast, training the GPU neural network required only a single NVIDIA RTX A4000 for 2 hours, encompassing 60 epochs (although it's worth noting that results ceased to improve after 30 epochs). It's worth mentioning that this hardware is considered outdated compared to the standard A100 typically used for substantial machine learning computations.

Regarding scaling, given the anticipated dominance of low-frequency disorder components, it may not be necessary to include all components to obtain a satisfactory approximation of the disorder. However, as more components become necessary, higher K resolution may be required to distinguish them effectively. For larger systems, KWANT scales approximately linearly in the generation process, but a larger system may also demand more components. In cases where all or a significant number of disorder components are needed, it might be more efficient to employ a convolutional upsampling decoder \cite{percebois2023reconstructing} to produce the disorder function. This approach would likely outperform our current method, which is optimized for handling smaller numbers of components.}






%Add discussion about resources used and expand upon the scaling question. 
%\begin{itemize}
%$\item Talk about low frequency dominance
%\item Talk about linear scaling with length
%\item Talk about how more resolution in K will be needed for more components
%\item Talk specifics of computation done.
%\item Talk about alternative decoder output method
%\end{itemize}



\section{Additional results}
\label{S:Add}
This section presents additional plots of numerical results.{\color{red} We provide the 10 disorder potentials and their corresponding conductances for $V_{\text{Bias}}$ vs. $B_x$, conductances for} $\mu$ vs. $B_x$ and $T_{IV}$ plots {\color{red}all} for both the input and prediction Y realizations. We include the conductance plots because the machine learning model utilizes $\mu$ vs. $B_x$ as its main input during the training process. The $T_{IV}$ plots demonstrate the ML model's capability to predict $T_{IV}$ solely based on conductance measurements. Moreover, we provide the conductance and $T_{IV}$ results for a pristine sample, which readers may find useful for comparison.


\begin{figure*}[t]
     \centering
        \begin{subfigure}[b]{0.95\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/YFourier10.png}
         \caption{}
         \label{fig:5a}
     \end{subfigure}
         \begin{subfigure}[b]{0.95\linewidth}
         \centering
          \includegraphics[width=\textwidth]{10DisorderResults/Y10.png}
         \caption{}
         \label{fig:5b}
     \end{subfigure}
     \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=0V.png}
         \caption{}
         \label{fig:5c}
     \end{subfigure}
          \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=1V.png}
         \caption{}
         \label{fig:5d}
     \end{subfigure}
          \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=2V.png}
         \caption{}
         \label{fig:5e}
     \end{subfigure}
          \begin{subfigure}[b]{0.48\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=3V.png}
         \caption{}
         \label{fig:5f}
     \end{subfigure}
     \caption{{\color{red}Representative samples of 10 disorder potential components neural network test input and predictions. (a) The discrete cosine transformed components of the disorder potential for 4 different samples and their respective predictions. (b) Disorder potentials in real space with deterministic modification due to boundary effects. In (c-f) the first row is $G_{LL}$, $G_{RR}$, $G_{LR}$ and $G_{RL}$ conductance measurements expected from a input disorder potential, and the second row is conductance measurements from the corresponding predicted disorder potential. Each of (c-f) are different disorder potential realizations, shown in (a). The conductance measurements are plotted for different values of $V_{\text{Bias}}$ (in meV) and $B_x$ (in T).   For this model $\alpha=8 meV/nm$ is fixed. The topological invariant corresponding to this profile can be seen in Fig. S6. The disorder amplitude and correlation length for each realization was $1.5$meV and 3 sites respectively. These are plotted for $\mu=0$.}}
     \label{fig:dVB2}
\end{figure*}

\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/Ex2Gs5_dr=0.png}
         \caption{}
         \label{fig:S1c}
     \end{subfigure}
          \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/Ex2Gs5_dr=1.png}
         \caption{}
         \label{fig:S1d}
     \end{subfigure}
          \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/Ex2Gs5_dr=2.png}
         \caption{}
         \label{fig:S1e}
     \end{subfigure}
          \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/Ex2Gs5_dr=3.png}
         \caption{}
         \label{fig:S1f}
     \end{subfigure}
     \caption{Representative samples of 5 disorder potential components and $\alpha$ neural network test input and predictions. In (a-d) the first row is $G_{LL}$, $G_{RR}$, $G_{LR}$ and $G_{RL}$ conductance measurements expected from a input disorder potential, and the second row is conductance measurements from the corresponding predicted disorder potential. Each of (a-d) is a different Y realization, shown in Fig. \ref{fig:D1}. The conductance measurements are plotted for different values of $\mu$ (in meV) and $B_x$ (in T). The topological invariant corresponding to this profile can be seen in Fig. \ref{fig:VIT1}. The disorder amplitude and correlation length for each realization was 1.5meV and 3 sites respectively. These plots use $V_{\text{Bias}}=0$.}
     \label{fig:DC1}
\end{figure*}
\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=0.png}
         \caption{}
         \label{fig:S2c}
     \end{subfigure}
          \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=1.png}
         \caption{}
         \label{fig:S2d}
     \end{subfigure}
          \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=2.png}
         \caption{}
         \label{fig:S2e}
     \end{subfigure}
          \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/Ex2Gs10_dr=3.png}
         \caption{}
         \label{fig:S2f}
     \end{subfigure}
     \caption{Representative samples of 10 disorder potential components neural network test input and predictions. In (a-d) the first row is $G_{LL}$, $G_{RR}$, $G_{LR}$ and $G_{RL}$ conductance measurements expected from a input disorder potential, and the second row is conductance measurements from the corresponding predicted disorder potential. Each of (a-d) are different disorder potential realizations, shown in Fig. \ref{fig:dVB2}a. The conductance measurements are plotted for different values of $\mu$ (in meV) and $B_x$ (in T). For this model $\alpha=8 \text{meV/nm}$ is fixed. The topological invariant corresponding to this profile can be seen in Fig. \ref{fig:VIT2}. The disorder amplitude and correlation length for each realization was 1.5meV and 3 sites respectively. These plots use $V_{\text{Bias}}=0$.}
     \label{fig:rDC2}
\end{figure*}
\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{5DisorderResults/TIV5.pdf}
         \caption{}
         \label{fig:9a}
     \end{subfigure}
     \caption{Representative samples of the topological invariant ($T_{IV}$) for 5 disorder potential components and $\alpha$ neural network test input and predictions. The first row is $T_{IV}$ resulting from a input disorder potential, and the second row is from the corresponding predicted disorder potential.  Each column are the different disorder potential realizations, shown in Fig. 3. The dotted red line corresponds to the conductance profiles in Fig. 2.  The topological invariant is plotted for different values of $\mu$ (in meV) and $B_x$ (in T).}
     \label{fig:VIT1}
\end{figure*}

\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{10DisorderResults/TIV10.pdf}
         \caption{}
         \label{fig:S3a}
     \end{subfigure}
     \caption{Representative samples of the topological invariant ($T_{IV}$) for 10 disorder potential components neural network test input and predictions. The first row is $T_{IV}$ resulting from a input disorder potential, and the second row is from the corresponding predicted disorder potential. Each column are the different disorder potential realizations, shown in Fig. \ref{fig:dVB2}a. The dotted red line corresponds to the conductance profiles in Fig. \ref{fig:dVB2}b-e.  The topological invariant is plotted for different values of $\mu$ (in meV) and $B_x$ (in T).}
     \label{fig:VIT2}
\end{figure*}


\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\textwidth]{PristineResults/PristineTIValpha=8.png}
         \caption{}
         \label{fig:S4a}
     \end{subfigure}
    \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{PristineResults/Pristine2Gsalpha=8.png}
         \caption{}
         \label{fig:S4b}
     \end{subfigure}
     \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{PristineResults/Exmu=0Pristine2Gsalpha=8V.png}
         \caption{}
         \label{fig:S4c}
     \end{subfigure}
      \begin{subfigure}[b]{0.9\linewidth}
         \centering
         \includegraphics[width=\textwidth]{PristineResults/Exmu=0pt3Pristinealpha=8V.png}
         \caption{}
         \label{fig:S4d}
     \end{subfigure}
     \caption{Pristine sample ($V_{\text{dis}}(x)=0$) topological invariant ($T_{IV}$) and conductance measurements. (a) The topological invariant and (b) Conductance measurements are plotted for different values of $\mu$ (in meV) and $B_x$ (in T) at $V_{Bias}=0$. Conductance measurements at (c) $\mu=0$ and (d) $\mu=0.3$ meV are plotted for different values of $V_{\text{Bias}}$ (in meV) and $B_x$ (in T).  The plots held fixed $\alpha=8 \text{meV/nm}$.}
     \label{fig:VIT}
\end{figure*}

\clearpage
\putbib
\end{bibunit}
